Line Failure Localization of Power Networks Part II: Cut Set Outages

Transmission line failure in power systems prop-agate non-locally, making the control of the resulting outages extremely difficult. In Part II of this paper, we continue the study of line failure localizability in transmission networks and characterize the impact of cut set outages. We establish a Simple Path Criterion, showing that the propagation pattern due to bridge outages, a special case of cut set failures, are fully determined by the positions in the network of the buses that participate in load balancing. We then extend our results to general cut set outages. In contrast to non-cut outages discussed in Part I whose subsequent line failures are contained within the original blocks, cut set outages typically impact the whole network, affecting the power flows on all remaining lines. We corroborate our analytical results in both parts using the IEEE 118-bus test system, in which the failure propagation patterns exhibit a clear block-diagonal structure predicted by our theory, even when using full AC power flow equations.

==> across_bridge_proof.tex <==
If $\hat{e}$ is a bridge, then since no simple loop can contain a bridge, the Simple Loop Criterion implies that $K_{\hat{e}e}=0$.

If $\hat{e}$ is not a bridge, without loss of generality, we can assume $e$ is within $\calN_1$ and $\hat{e}$ is within $\calN_2$. Since $\calP$ is a tree-partition, any path starting from a node in $\calN_1$ and ending at a node in $\calN_2$ must pass through all bridges in the path in the reduced graph $\calG_\calP$ (see Part I for more details of this reduced graph) from $\calN_1$ to $\calN_2$. As a result, any loop containing both $e$ and $\hat{e}$ must pass through these bridges at least twice, and thus is not simple. By the Simple Loop Criterion, we then know that $K_{\hat{e}e}=0$. \qed

==> basic.tex <==
\begin{figure}
\centering
\iftoggle{isarxiv}{
\includegraphics[width=0.325\textwidth]{tree_partition.png}
}{
\includegraphics[width=0.325\textwidth]{figs/tree_partition.png}
}
\caption{The construction of $\calG_\calP$ from $\calP$.}\label{fig:tree_partition}
\end{figure}

%The tree partition of a power system graph has emerged as a powerful tool in cascading failure analysis. 
The idea of tree partition for analyzing cascading failure was first introduced in \cite{guo2017monotonicity}. Here, we define the tree partition, discuss its uniqueness and show that the ``finest'' tree partition of a general graph can be computed in linear time.

%To start with, we first formally define the concept of tree partition. 
For a power network $\calG=(\calN,\calE)$, a collection $\calP=\set{\calN_1,\calN_2,\cdots, \calN_k}$ of subsets of $\calN$ is said to form a \emph{partition} of $\calG$ if $\calN_i\cap\calN_j=\emptyset$ for $i\neq j$ and $\cup_{i=1}^k \calN_i=\calN$. For any partition, we can define a reduced multi-graph $\calG_\calP$ from $\calG$ as follows. First, we reduce each subset $\calN_i$ to a super node (see Fig.~\ref{fig:tree_partition}). The collection of all super nodes forms the node set for $\calG_\calP$. Second, we add an undirected edge connecting the super nodes $\calN_i$ and $\calN_j$ for each pair of $n_i, n_j\in\calN$ with the property that $n_i\in\calN_i$, $n_j\in\calN_j$ and $n_i$ and $n_j$ are connected in $\calG$. Note that multiple ledges are added when multiple pairs of such $n_i,n_j$ exist. Unlike the graph $\calG$ to which we assign an arbitrary orientation (and thus is a directed graph), the reduced multi-graph $\calG_\calP$ is undirected.

\begin{defn}
A partition $\calP=\set{\calN_1,\calN_2,\cdots,\calN_k}$ of $\calG$ is said to be a \textbf{tree partition} if the reduced graph $\calG_\calP$ forms a tree.
\end{defn}

\begin{defn}
Given a tree partition $\calP=\set{\calN_1,\calN_2,\cdots,\calN_k}$, the sets $\calN_i$ are called the \textbf{regions} of $\calP$. An edge $e=(w,z)$ with both endpoints inside $\calN_i$ is said to be \textbf{within} $\calN_i$. If $e$ is not within $\calN_i$ for any $i$, then we say $e$ forms a \textbf{bridge}\footnote{We remark that our definition of bridges agrees with the classical definition of bridges in graph theory (i.e., the removal of any such edge disconnects the original graph) in the sense that if the tree partition $\calP$ is irreducible (see Definition \ref{defn:irreducible} later) any bridge defined in our sense is a bridge in the classical sense, and vice versa.}.
\end{defn}

Tree partitions of a power network $\calG$ are generally not unique. For instance, one can always collapse $\calG$ into a single region with the partition $\calP_0=\set{\calN}$, which is a trivial tree partition of $\calG$. This yields a different tree partition for the graph shown in Fig.~\ref{fig:tree_partition}. Nevertheless, if we require the tree partition to be as ``fine'' as possible, such a partition is unique.

More concretely, given a graph $\calG$, we define a partial order $\succeq$ over the set of all tree partitions of $\calG$ (which is nonempty as it always contains the trivial partition $\calP_0$) as follows: For two tree partitions $\calP^1=\set{\calN_1^1,\calN_2^1,\cdots,\calN_{k_1}^1}$ and $\calP^2=\set{\calN_1^2,\calN_2^2,\cdots,\calN_{k_2}^2}$, we say $\calP^1$ is \emph{finer} than $\calP^2$, denoted as $\calP^1\succeq \calP^2$, if for any $i=1,2,\ldots, k_1$, there exists some $j(i)\in \set{1,2,\ldots, k_2}$ such that $\calN_i^1\subset \calN_{j(i)}^2$. That is, $\calP^1$ is finer than $\calP^2$ if each region in $\calP^1$ is contained in some region in $\calP^2$ (see Fig.~\ref{fig:partition_order}). It is routine to check that $\succeq$ defines a partial order over all possible tree partitions of $\calG$.

\begin{defn}\label{defn:irreducible}
A tree partition $\calP$ of $\calG$ is said to be \textbf{irreducible} if $\calP$ is maximal with respect to the partial order $\succeq$.
\end{defn}

In other words, an irreducible tree partition $\calP$ of $\calG$ is a partition that cannot be reduced to a finer tree partition.

\begin{prop}\label{prop:unique_irreducible}
For any graph $\calG$, there exists a unique irreducible tree partition.
\end{prop}
\iftoggle{isreport}{
See Appendix \ref{proof:uniqueness} for a proof.
}{
See our online report for a proof \cite{report}.
}

\begin{figure}[t]
\centering
\iftoggle{isarxiv}{
\includegraphics[width=.275\textwidth]{partition_order.png}
}{
\includegraphics[width=.275\textwidth]{figs/partition_order.png}
}
\caption{An illustration of the partial order $\succeq$ over tree partitions. The partition $\calP^1=\set{\calN_1^1, \calN_2^2, \calN_3^1, \calN_4^1}$ is finer than $\calP^2=\set{\calN_1^2, \calN_2^2}$.}\label{fig:partition_order}
\end{figure}
We remark that our proof of Proposition \ref{prop:unique_irreducible} not only shows that the irreducible tree partition of $\calG$ is unique, but also implies that the problem of computing this unique irreducible tree partition reduces to finding all bridges of $\calG$. As a result, we can adapt Tarjan's bridge-finding algorithm \cite{tarjan1974note} to devise an algorithm that computes the irreducible tree partition of $\calG$ in $O(n+m)$ time. This is summarized in Algorithm \ref{alg:tree_partition}. Interested readers are referred to the proof of Proposition \ref{prop:unique_irreducible} in\iftoggle{isreport}{ Appendix \ref{proof:uniqueness}}{~\cite{report}} for more details on the algorithm.

\begin{algorithm}
\caption{Irreducible Tree Partition Finding Algorithm}\label{alg:tree_partition}
\begin{algorithmic}[1]
    \STATE Execute Tarjan's bridge-finding algorithm \cite{tarjan1974note} on $\calG=(\calN,\calE)$ to compute the set of bridges $\calE_b$.
    \STATE Remove edges in $\calE_b$ from $\calE$ to form the partitioned graph $(\calN, \calE\bs\calE_b)$.
    \STATE Breadth-first search on the partitioned graph $(\calN,\calE\bs\calE_b)$ to compute its set of connected components $\calP:=\set{C_1, C_2, \ldots, C_k}$. Return $\calP$.
     \end{algorithmic}
\end{algorithm}

To summarize, we have shown that each graph $\calG$ has a unique irreducible tree partition, which can be computed in linear time. Thus, to simplify the terminology, whenever we say the tree partition of $\calG$ in the sequel, we always refer to its irreducible partition. 

==> bridge_prop_general_proof.tex <==
\begin{figure}
\centering
\iftoggle{isarxiv}{
\includegraphics[width=.45\textwidth]{localized_graph.png}
}{
\includegraphics[width=.45\textwidth]{figs/localized_graph.png}
}
\caption{The localized graph $\calG_{\calN_1}$. $\calN_t$ is the imaginary bus containing $e$ and $\calN_{1,i}$'s are remaining imaginary buses. The power adjustments from the power balance rule $\calR$ are shown near each participating bus in reaction to a power loss of $M$.}\label{fig:localized}
\end{figure}
By merging two tree-partition regions if necessary, we can assume $\hat{e}$ belongs to a certain tree-partition region, say $\calN_1$. Let $n_1,n_2,\cdots, n_l$ be the set of participating buses in $\calN_1$. By collapsing all regions other than $\calN_1$, we can define a ``localized'' graph $\calG_{\calN_1}$ centered around $\calN_1$ as shown in Fig.~\ref{fig:localized}, with the following constructions: (a) For each bridge $b$ incident to $\calN_1$, we create an imaginary bus that aggregates all injections inside all tree-partition regions that can be reached by $\calN_1$ through $b$ \emph{before} $e$ is tripped, and this imaginary bus is connected to $\calN_1$ via the corresponding bridge $b$. (b) If $e$ is not directly incident to $\calN_1$, then $e$ must connect two regions that are collapsed to a common imaginary bus, say $\calN_t$. If $e$ is incident to $\calN_1$ and its end point in $\calN_1$ is $w$, then we let $\calN_t$ be an additional imaginary bus that is connected to $w$ to mimic the edge $e$ (that is, before $e$ is tripped this imaginary bus $\calN_t$ supplies power $f_e$ towards $w$ and after $e$ is tripped, $\calN_t$ loses all its injection; moreover, the edge connecting $\calN_t$ to $n_e$ has susceptance $B_e$). Denote other imaginary buses as $\calN_{1,1},\calN_{1,2},\cdots, \calN_{1,q}$. 

Without loss of generality, let us assume because of the tripping of $e$, the aggregate power in $\calD$ is in shortage of $M:=f_e$. Then the enforcement of the power balance rule $\calR$ would increase the power injection at each participating bus in $\calD$, which translates to the power adjustment as demonstrated in Fig.~ \ref{fig:localized}. Specifically, the injection at $\calN_t$ would drop by $\alpha_{\calN_t}M$ as the power flow from $e$ is lost (the drop is generally not $M$ unless $e$ is directly incident to $\calN_1$); the injections at $\calN_{1,1},\calN_{1,2}, \cdots, \calN_{1,q}$ increase by $\alpha_{\calN_{1,i}} M$; and injections at the participating buses $n_1,n_2,\cdots, n_l$ in $\calN_1$ increase by $\alpha_{n_i}M$. In other words, by rebalancing power according to the rule $\calR$, we effectively shift the injections from $\calN_t$ to $\calN_{1,1},\calN_{1,2}, \cdots, \calN_{1,q}$ and $n_1,n_2,\cdots, n_l$.

Let the set of edges in $\calG_{\calN_1}$ be $\calE_1$. Pick $\calN_t$ to be the slack bus in this localized graph $\calG_{\calN_1}$ and define an index set
$$
\calI:=\set{\calN_{1,1},\calN_{1,2}, \cdots, \calN_{1,q}, n_1,n_2,\cdots, n_l}.
$$
Write $\hat{e}=(w,z)$. For any $i\in\calI$, let $g^{i}(B)$ be the following polynomial in line susceptances $(B_e:e\in\calE_1)$:
$$
\sum_{E\in\calT_{\calE_1}\paren{\set{i,w},\set{\calN_t,z}}}\chi(E) - \sum_{E\in\calT_{\calE_1}\paren{\set{i,z},\set{\calN_t,w}}}\chi(E),
$$
where $\calT_{\calE_1}\paren{\calN_1,\calN_2}$ is the set of spanning forests of $\calG_{\calN_1}$ consisting of exactly two trees that contain $\calN_1$ and $\calN_2$ respectively. By our graphical representation of the generation shift sensitivity factor from Part I, the branch flow change on $\hat{e}$ coming from the power shift from $\calN_t$ with amount $\alpha_iM$ towards $i$ is given by
$$
\Delta f^{i}_{\hat{e}}=\alpha_{i}M \times \frac{g^{i}(E)}{\sum_{E\in\calT_{\calE_1}}\chi(E)},
$$
where $\calT_{\calE_1}$ denotes the set of all spanning trees of $\calG_{\calN_1}$. Set
$$
g(B):=\sum_{i\in\calI}\alpha_{i}g^{i}(B).
$$
By linearity, we have
$$
\Delta f_{\hat{e}}=M\times \frac{g(B)}{\sum_{E\in\calT_{\calE_1}}\chi(E)}.
$$

If $g(B)\neq 0$, then we can find at least one $i$ such that $\calT_{\calE_1}\paren{\set{i,w},\set{\calN_t,z}}$ or $\calT_{\calE_1}\paren{\set{j,z},\set{\calN_t,w}}$ is nonempty. Without loss of generality, assume that
$$
\calT_{\calE_1}\paren{\set{i,w},\set{\calN_t,z}}
$$
is nonempty. Any element in $\calT_{\calE_1}\paren{\set{i,w},\set{\calN_t,z}}$ contains two trees containing $\set{i,w}$ and $\set{\calN_t,z}$ respectively, and thus induces one path from $w$ to $i$ and another path from $\calN_t$ to $z$. By adjoining $(w,z)$ to these two paths, we can create a path from $i$ to $\calN_t$ that contains $\hat{e}$. It is easy to see that this path induces a path in the original graph $\calG$ between $u$ and a certain participating bus $j$. Therefore, $\Delta f_{\hat{e}}\neq 0$ only if there exists $j\in\calN_\calR$ such that there is a path in $\calD$ from $u$ to  a participating bus $j$ containing $\hat{e}$.

On the other hand, if there is a path $P$ in $\calD$ from $u$ to a participating bus $j$ containing $\hat{e}$, we claim $g(B)$ is not identically zero. Indeed, by a similar argument to the proof of Proposition \ref{prop:same_region}, we know that for any $i,j\in\calI$ (including the case $i=j$), the following is true:
$$
\calT_{\calE_1}\paren{\set{i,w},\set{\calN_t,z}}\cap \calT_{\calE_1}\paren{\set{j,z},\set{\calN_t,w}}=\emptyset.
$$
As a result, a term in $g^i(B)$ with positive coefficient  is never canceled by a term in $g^j(B)$ with negative coefficient, and vice-versa. Therefore, to show $g(B)$ is not identically zero, it suffices to show at least one term of $g^i(B)$ is not identically zero.

To do so, note that by removing $\hat{e}$ from $P$, we can create a path from $u$ to one endpoint of $\hat{e}$, say $w$, and another path from $z$ to $j$. This implies that in the localized graph Fig.~\ref{fig:localized} we have a path from $\calN_t$ to $w$ and another path from $z$ to some $i\in\calI$. By iteratively adding edges, these two paths can be extended to an element in  $\calT_{\calE_1}\paren{\set{j,z},\set{\calN_t,w}}$, which contributes to a term of $g^i(B)$ that is not identically zero.

Again by the classical algebraic geometry result asserting the root set of any polynomial that is not identically zero has Lebesgue measure zero \cite{federer1969geometric}, and from to the absolute continuity of $\mu$ it follows that
$$
\mu\paren{\Delta f_{\hat{e}}=0}=\calL_m\paren{g(B+\omega)=0}=0
$$
and thus $\mu\paren{\Delta f_{\hat{e}}\neq 0} = 1$. \qed

==> bridge_prop_proof.tex <==
If $\hat{e}$ is a bridge, denote the two connected components of $\calD$ after removing $\hat{e}$ as $\calD_1$ and $\calD_2$, and without loss of generality assume $\calD_1$ is originally connected to $e$ in $\calG$. It is easy to see that the branch flow change on $\hat{e}$ is given by
$$
\Delta f_{\hat{e}} = \sum_{j\in \calD_2}(\Delta p_\calD)_j \neq 0,
$$
where the last $\neq$ is because the grid is participating and thus all tree-partition regions in $\calD_2$ would adjust their injections (in the same ``direction'' as $\alpha_j$'s are positive). 

If $\hat{e}$ is not a bridge, then Lemma \ref{lemma:participating_region} implies $\mu(\Delta f_{\hat{e}}\neq 0) = 1$. \qed

==> dirac.tex <==
In our discussions on the perturbation $\mu$, we have assumed $\mu$ to be absolutely continuous with respect to the Lebesgue measure $\calL_m$ on $\R^m$. The main purpose of this assumption is to simplify the presentation. In this appendix, we demonstrate for Proposition \ref{prop:same_region} how our results can be generalized when this absolute continuity assumption is not imposed.

Let $\Omega:=\set{\omega: f(B+\omega)=0, \mu(\set{\omega}) > 0}$ be the set of Dirac masses of $\mu$ at which the polynomial $f$ (as defined in the Proof of Proposition \ref{prop:same_region}) vanishes. It is easy to show that $\Omega$ is a countable set and hence measurable (thus $\mu(\Omega)$ is meaningful). From the proof of Proposition \ref{prop:same_region}, it is not hard to see the following:
\begin{prop}
Consider a power network $\calG$ with susceptance perturbation $\mu$ and let $e,\hat{e}$ be two distinct edges within the same cell.  We have:
$$
\mu\paren{K_{\hat{e}e}\neq 0} = 1 - \mu(\Omega).
$$
\end{prop}

All of our results involving $\mu$ can be generalized in this way.

\qed

==> effective_reactance.tex <==
The Laplacian matrix $L$ appears in circuit analysis as the admittance matrix (with a different weight), which explicitly relates the voltage and current vector in an electrical network \cite{dorfler2013kron}. In particular, given a networked resistors, it is shown in \cite{dorfler2013kron} that the effective resistance between two nodes $i$ and $j$ can be computed as
\begin{equation}\label{eqn:prem_effective_reactance}
R_{ij}:=L^\dagger_{ii}+L^\dagger_{jj}-L^\dagger_{ij}-L^\dagger_{ji}
\end{equation}
where $L^\dagger$ is the Penrose-Moore pseudoinverse of $L$. Following a similar calculation, we can show that \eqref{eqn:prem_effective_reactance} also gives the effective reactance between the buses $i$ and $j$ in a power system. That is, assuming we connect the buses $i$ and $j$ to an external probing circuit, when there is no other injection in the network, the power flow $f_{ij}$ (from the external circuit) into bus $i$ and out from bus $j$ (into the external circuit) is given as
$$
f_{ij}=\frac{\theta_i-\theta_j}{R_{ij}}
$$
and therefore the network can be equivalently reduced to a single line with reactance $R_{ij}$. If $(i,j)\in\calE$, that is $i$ and $j$ are directly connected, then physical intuition suggests
$$
R_{ij} < X_{ij}
$$
where $X_{ij}:= 1/B_{ij}$ is the reactance of line $(i,j)$, as connections from the network should only decrease the overall reactance. We show in Section \ref{section:prem_inversion} that $X_{ij}-R_{ij}$ also carries graphical meaning, proving its nonnegativity rigorously.

==> intro-v1.tex <==
In Part I of this paper \cite{part1}, we establish the spectral representation of power redistribution that precisely captures the Kirchhoff's Law in terms of the distribution of different families of subtrees in the transmission network. This new representation motivates a novel approach to localize cascading failures in power systems.
% : more specifically, we propose switching off a few carefully chosen transmission lines and creating in this way a finer network tree partition.

\textbf{Contributions of Part II of this paper:} \emph{We prove that the tree partition proposed in Part I provides a precise analytical characterization of line failure localizability, and we show how to use this characterization to mitigate failure cascading by switching off a small number of carefully chosen transmission lines and creating in this way a finer network tree partition.} Our results rigorously establish the informal intuition of the power community that failures cannot cross bridges, and reveal a finer-grained concept that encodes more precise information on failure propagation within tree-partition regions. This work builds on the recent work focused on the line outage distribution factor, e.g., \cite{soltan2015analysis, guo2017monotonicity}, and shows that tree partition is a particularly useful representation of this factor, one that captures many aspects of how line failures can cascade.

The formal characterization of localizability in the case of a single line failure is given in Theorem \ref{thm:summary} of Section \ref{section:summary}, which summarizes the technical results in Sections \ref{section:non-bridge} and \ref{section:bridge}.  In particular, in Section \ref{section:non-bridge}, we characterize power redistribution after the tripping of a single non-bridge line and show that the impact of such failures only propagates within well-defined components, which we refer to as cells, inside the tree-partition regions. In Section \ref{section:bridge}, we consider the failure of a single bridge line and prove that, in normal operating conditions, such a failure propagates globally across the network and impacts the power flows on all transmission lines.

In Section \ref{section:multi_line}, we extend Theorem \ref{thm:summary} to the case of multiple simultaneous line failures, and show that the aggregate impact of such failure consists of two parts: (a) a part from power redistribution that generalizes the case of a single non-bridge failure, and such impact can be decomposed in accordance to the cells where the failures occur; (b) a part from power balancing rule that generalizes the case of a single bridge failure and captures how the system handles disconnected components. In order to prove these results, we depend on properties of the tree partition proved in Part I \cite{part1}. Further, we make use of the block decomposition of tree-partition regions to completely eliminate simple loops containing edges among distinct cells, which from the Simple Loop Criterion in Part I \cite{part1} guarantees failure localization. Lastly, we apply classical techniques from algebraic geometry to address potential pathological system specifications.

The characterizations we provide in Theorem \ref{thm:summary} and Section \ref{section:multi_line} yield many insights for the planning and management of power systems and further suggests a new approach for mitigating the impact of cascading failures. Specifically, our characterization highlights that switching off certain transmission lines with respect to real-time injection profiles can lead to more, smaller regions/cells (and hence a finer tree partition of the grid).  This localizes line failures better and thus makes the grid more robust against large-scale blackouts. 
In Section \ref{section:case_study}, we illustrate this approach using the IEEE 118-bus test network. We demonstrate that switching off only a negligible portion of transmission lines can lead to significantly better control of cascading failures.  Further, we highlight that this happens without significant increase in line congestion across the network. 

\slow{Highlight this somewhere about simultaneous line failures: 
In particular, the fact that $K_{\hat ee'} \neq 0$ and $ \left( H_i \right)_{e'e}\neq 0$ (a.s.) if the remaining line $\hat e$ and 
 the outaged lines $e, e'$ are in the same cell $\calC_i$ means that every line failure will impact the power flows on every
remaining line (only) within the same cell.}

\slow{Comment more explicitly localization results of non-cut set failures vs intuition that \emph{all} bridge flows in any
tree partition will remain unchanged after a non-cut set failure.   Results rigorous prove the following:
\begin{itemize}
\item Failure (single or multi-line) in a cell will impact flows on lines within the same cell only.  This is intuitive in retrospect.
\item Failure (single or multi-line) in a cell will impact flows on \emph{every} line within the same cell (a.s.).  This is not intuitive to the best
	of our knowledge. Result also reveal how the impact of a bridge failure propagates globally and how this depends on the design of
	balancing rules and topological structure of injections participating in rebalancing.
\end{itemize}
Other finer details: 
\begin{itemize}
\item Localization is not at the level of tree-partition regions, but on a finer structure we call cells within each region.
\item Simple Loop Criterion that is easy to apply in practice that summarizes the impact (for single-line failure \emph{only}?).
\item Various explicit formulae on flow changes on remaining lines that can be useful for applications such as contingency analysis.
\end{itemize}
}


\slow{Re-organize to put single-line (THeorem 2) and multi-line case (Theorem 13, and implication of Propositions 14, 15) on the same footing?
}



==> localization_proof.tex <==
By Theorem \ref{thm:multi_line_no_cut}, for any $\mathfrak{n}$, if $\calB(\mathfrak{n})\subset \calC$ and $\calF(\mathfrak{n})$ is a non-cut set of $\calG(\mathfrak{n})$, then only edges within $\calC$ can potentially have a new branch flow, and therefore $\calF(\mathfrak{n})\subset \calC$. If $\calF(\mathfrak{n})$  is a non-cut set of  $\calG(\mathfrak{n})$, then $\calB(\mathfrak{n}+1)=\calB(\mathfrak{n}) \cup \calF(\mathfrak{n})$ is a non-cut set of $\calG(\mathfrak{n}+1)$. The desired result thus follows by induction.

\qed

==> model.tex <==
We use the graph $\calG=(\calN,\calE)$ to describe a power transmission network, where $\calN=\set{1,\ldots, n}$ is the set of buses and $\calE\subset\calN \times \calN$ is the set of transmission lines. The terms bus/vertex and line/edge are used interchangeably. An edge in $\calE$  between vertices $i$ and $j$ is denoted either as $e$ or $(i,j)$. We assume $\calG$ is connected and simple, and assign an arbitrary orientation over $\calE$ so that if $(i,j)\in\calE$ then $(j,i)\notin\calE$. The line susceptance of $e$ is denoted as $B_e$ and the branch flow on $e$ is denoted as $P_e$. The susceptance matrix is defined to be the diagonal matrix $B=\diag(B_e: e\in\calE)$. 

We denote the power injection and phase angle at bus $i$ as $p_i$ and $\theta_i$, and use $n$ and $m$ to denote the number of buses and transmission lines in $\calG$. The vertex-edge incidence matrix of $\calG$ is the $n\times m$ matrix $C$ defined as
$$
C_{ie}=\begin{cases}
  1 & \text{if vertex }i\text{ is the source of }e\\
  -1 & \text{if vertex }i\text{ is the target of }e\\
  0 &\text{otherwise.}
\end{cases}
$$
With the above notation, the DC power flow model can be written as
\begin{subequations}\label{eqn:dc_model}
\begin{IEEEeqnarray}{rCl}
	p&=&CP \label{eqn:flow_conservation}\\
	P&=&BC^T\theta, \label{eqn:kirchhoff}
\end{IEEEeqnarray}
\end{subequations}
where \eqref{eqn:flow_conservation} is the flow conservation constraint and \eqref{eqn:kirchhoff} is Kirchhoff's and Ohm's Laws. The slack bus phase angle in $\theta$ is typically set to $0$ as a reference to other buses. With this convention, the DC model \eqref{eqn:dc_model} has a unique solution $\theta$ and $P$ for each injection vector $p$ such that $\sum_{j\in\calN}p_j=0$.

\begin{figure}
\centering
\iftoggle{isarxiv}{
\includegraphics[width=.275\textwidth]{spanning_forest.png}
}{
\includegraphics[width=.275\textwidth]{figs/spanning_forest.png}
}
\caption{An example element in $\calT(\calN_1,\calN_2)$, where circles correspond to elements in $\calN_1$ and squares correspond to elements in $\calN_2$. The two trees containing $\calN_1$ and $\calN_2$ are highlighted as solid lines.}\label{fig:spanning_forest}
\end{figure}

When a line $e$ is tripped, the power flow redistributes according to the DC model \eqref{eqn:dc_model} on the newly formed graph $\calG'=(\calN,\calE\bs\set{e})$. If $\calG'$ is still connected, then the branch flow change on a line $\hat{e}$ is given as
$$
	\Delta P_{\hat{e}} = P_e\times K_{e\hat{e}},
$$
where $K_{e\hat{e}}$ is the \emph{line outage distribution factor} \cite{wood1996generation} from $e$ to $\hat{e}$. It is known that this distribution factor is independent of the original power injection $p$ and can be computed from the matrices $B$ and $C$ \cite{wood1996generation}.

If the new graph $\calG'$ is disconnected, then it is possible that the original injection $p$ is no longer balanced in the connected components of $\calG'$. Thus, to compute the new power flow, a certain power balance rule $\calB$ needs to be applied. Several such rules have been proposed and evaluated in literature based on load shedding or generator response \cite{soltan2015analysis,bernstein2014power,bienstock2010n-k,bienstock2011control,bernstein2014vulnerability}. In this work, we do not specialize to any such rule and instead opt to identify the key properties of these rules that allow our results to hold. With this more abstract approach, we can characterize the power flow redistribution under a class of power balance rules. 

The line outage distribution factor has been extensively studied in previous work, and we make use of some important properties from this literature. In \cite{guo2017monotonicity}, by studying the spectrum of the graph Laplacian, a formula for $K_{e\hat{e}}$ is given in terms of the graph structure of $\calG$. This formula plays a central role in proving almost all of the results in this paper, and we thus restate it here. To do so, we need some more notation. For two subsets of vertices $\calN_1, \calN_2\subset\calN$, let $\calT(\calN_1, \calN_2)$ be the set of spanning forests of $\calG$ consisting of \emph{exactly} two trees that contain $\calN_1$ and $\calN_2$ respectively\footnote{This definition does not require $\calN_1$ and $\calN_2$ to be disjoint, and $\calT(\calN_1, \calN_2)$ is understood to be empty when $\calN_1\cap\calN_2\neq \emptyset$.  See \cite{guo2017monotonicity} for more discussions.}. See Fig.~\ref{fig:spanning_forest} for an illustration. Given a set $E\subset\calE$ of lines, we assign a weight to $E$ by multiplying the susceptances over all lines in $E$
$$
\chi(E):=\prod_{e\in E}B_e
$$
and denote the set of all spanning trees of $\calG$ with edges only from $E$ by $\calT_E$ (which can be empty if $E$ is too small). The following result from \cite{guo2017monotonicity} is used throughout this paper.
\begin{thm}\label{thm:redist_factor}
Let $e=(i,j), \hat{e}=(w,z)$ be edges such that the $\calG'=(\calN, \calE\bs\set{e})$ is connected. Then $K_{e\hat{e}}$ is given by
\begin{equation*}
B_{\hat{e}}\times\frac{\sum_{E\in \calT(\set{i,w},\set{j,z})}\chi(E)-\sum_{E\in \calT(\set{i,z},\set{j,w})}\chi(E)}{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\chi(E)}
\end{equation*}
\end{thm}
This result reflects Kirchhoff's Law in a precise way and shows that the impact of a line failure propagages through spanning forests inside $\calG$. Interested readers are directed to \cite{guo2017monotonicity} for a more detailed discussion.

==> multi_line_adjustment_proof.tex <==
Denote the original injection over $\calD$ by $p_\calD$, then after tripping $E$, the new injection in $\calD$ is $p_\calD+\Delta p_\calD$. Therefore, the new power flow is given by
$$
\tilde{f}_{\calD}=B_\calD C_{\calD}^TA_\calD (p_\calD+\Delta p_\calD).
$$
Since $B_\calD C_{\calD}^TA_\calD p_\calD$ is simply the power flow on $\calD$ after $E_\calD$ is tripped under the original injection $p_\calD$, we see that
$$
B_\calD C_{\calD}^TA_\calD p_\calD = f_\calD + K^{E_\calD}f_{\calE_\calD}.
$$
The desired result then follows. \qed

==> multi_line_label_proof.tex <==
Let $L^E:=C_E^TAC_E$. First we claim that if $e_i\in E_i$, $e_j\in E_j$ and $i\neq j$, then $L^E_{e_ie_j}=0$. To see this, note that 
$$
(B_EL^E)_{e_ie_j} = D_{e_i, e_j},
$$
where $D_{e_i, e_j}$ is the generation shift sensitivity factor from $e_j$ to $e_i$ (see Part I). It is easy to see that $D_{e_i,e_j}=0$ if and only if $K_{e_ie_j}=0$. As a result, if $e_i$ and $e_j$ are in different cells, then $D_{e_i,e_j}=0$. 

Since $I$ is diagonal, by permuting the edges according to the cells they belong to, the matrix $I-B_EL^E$ has the following block-diagonal form:
$$
\begin{bmatrix}
J_{1}& 0& \cdots& 0\\
0 & J_{2} & \cdots & 0\\
\vdots & \vdots & \ddots & \vdots\\
0 & 0 &\cdots & J_{k}
\end{bmatrix},
$$
where $J_{i}\in\R^{m_i\times m_i}$ for $i=1,2,\cdots, k$. Moreover, each $J_i$ is invertible since $I-B_EL^E$ is invertible (see \cite{StottAlsacAlvarado1985} for instance). This, in particular, implies that $(I-B_EL^E)^{-1}$ is of the form
$$
\begin{bmatrix}
H_{1}& 0& \cdots& 0\\
0 & H_{2} & \cdots & 0\\
\vdots & \vdots & \ddots & \vdots\\
0 & 0 &\cdots & H_{k}
\end{bmatrix},
$$
where $H_{i}\in\R^{m_i\times m_i}$ for $i=1,2,\cdots, k$.

Next, we consider $H_1$ and fix $e_1, e_2 \in \set{1, 2, \cdots, m_1}$ to be two edges in the cell $\calC_1$. Then,
$$
(H_1)_{e_1e_2}=\frac{\det(J_1^{e_1,e_2})}{\det(J_1)},
$$
where $J_1^{e_1,e_2}$ is the matrix obtained from $J_1$ by replacing the $e_1$-th column with a vector with value $1$ at $e_2$-th component and $0$ elsewhere. Set $J_1'$ to be the submatrix of $J_1$ obtained by removing the $e_1$-th column and $e_2$-th row from $J_1$. Then,
$$
\det(J_1^{e_1,e_2})=(-1)^{e_1+e_2}\det(J_1').
$$
The entries of $J_1'$ are of the form $1-D_{e_i,e_i}$ or $D_{e_i, e_j}$. Recall from Part I that for any pair of edges $e_i=(u,v), e_j=(w,z)$, we have $D_{e_i, e_j}$ be given by
%  \begin{IEEEeqnarray*}{rCl}
%&&\frac{B_{e_i}}{\sum_{E\in \calT_\calE}\chi(E)}\times\\
%&& \Bigg(\sum_{E\in \calT(\set{u,w},\set{v,z})}\chi(E)
%-\sum_{E\in \calT(\set{u,z},\set{v,w})}\chi(E)\Bigg).
%  \end{IEEEeqnarray*}
  \begin{IEEEeqnarray*}{rCl}
	&&\frac{B_{e_i}}{\sum_{F\in \calT_\calE}\chi(F)}\times\\
	&& \Bigg(\sum_{F\in \calT(\set{u,w},\set{v,z})}\chi(F)
	-\sum_{F\in \calT(\set{u,z},\set{v,w})}\chi(F)\Bigg).
\end{IEEEeqnarray*}
Note that we use $F$ to indicate the edge set of spanning forests, and set $E$ as the set of line failures.
Since all edges in $E_1$ are within the same cell, $D_{e_i, e_j}$ is not identically zero for any $e_i,e_j\in E_1$ (including the case $e_i=e_j$). We now show that $\det(J_1')$ is a polynomial in $B$ that is not identically zero. To do so, we first prove the following three technical lemmas:
\begin{lemma}\label{lemma:no_contain}
If $e_i\neq e_j$ are two different edges, then any term in the numerator of $D_{e_i,e_j}$ does not contain $B_{e_j}$.
\end{lemma}
\begin{proof}
The numerator of $D_{e_i,e_j}$ is given by the difference of
$$
   B_{uv}\sum_{F\in \calT(\set{u,w},\set{v,z})}\chi(F)
$$
and
$$
   B_{uv}\sum_{F\in \calT(\set{u,z},\set{v,w})}\chi(F).
$$
When $e_i\neq e_j$, for each element of $F\in\calT(\set{u,w},\set{v,z})$, adding $e_i=(u,v)$ to $F$ induces a spanning tree of $\calG$ that passes through $e_i=(u,v)$ but not $e_j=(w,z)$, and $d_F(u,w)<d_F(v,w)$, where $d_F(\cdot,\cdot)$ means the distance in terms of minimum number of hops in $F$. Conversely, for any spanning tree of $\calG$ that passes through $e_i=(u,v)$ but not $e_j=(w,z)$, and $d_F(u,w)<d_F(v,w)$, removing $e_i$ induces an element of $F\in\calT(\set{u,w},\set{v,z})$.
  
A similar argument also applies to $\calT(\set{u,z},\set{v,w})$. Therefore, the numerator of $D_{e_i,e_j}$ is exactly given as
  \begin{equation}\label{eqn:local_exp_formula}
  \sum_{F\in\calT_{e_i, - e_j}}\sign(F)\chi(F),
  \end{equation}
where $\calT_{e_i, - e_j}$ is the set of spanning trees of $\calG$ that pass through $e_i=(u,v)$ but not $e_j=(w,z)$, and
  $$
  \sign(F):=\begin{cases}
  1, &d_F(u,w) < d_F(v, w)\\
  -1,& d_F(u,w) \ge d_F(v,w).
  \end{cases}
  $$
In particular, $B_{e_j}$ does not appear in any of these terms.
\end{proof}
\begin{lemma}\label{lemma:contain}
If $e_i=e_j$, then the numerator of $D_{e_i,e_j}$ is 
$$
  \sum_{F\in\calT_{e_i}}\chi(F),
  $$
where $\calT_{e_i}$ consists of all spanning trees of $\calG$ that pass through $e_i$.
\end{lemma}
\begin{proof}
When $e_i=e_j$, $D_{e_i, e_j}/B_{e_i}$ reduces to the effective reactance of $e_i$, and the result then follows directly from Corollary 7 of Part I.
\end{proof}
\begin{lemma}\label{lemma:non_vanishing}
Let $g_1, g_2,\cdots, g_{l_1}$ and $h_1, h_2, \cdots, h_{l_2}$ be functions in $B$ of the form  $D_{e_i, e_j}$ with $e_i,e_j \in \calC_1$. Assume the $e_j$'s for $g_k$ are different over $k=1,2,\cdots, l_1$, and the $e_j$'s for $h_k$ are different over $k=1,2,\cdots, l_2$. Let $q_1$ be the number of $g_k$'s with $e_i=e_j$, and $q_2$ be the number of $h_k$'s with $e_i = e_j$. If $q_1\neq q_2$, then for any fixed $a_1, a_2\neq 0$, the function
$$
f(B):=a_1\prod_{k=1}^{l_1}g_k + a_2\prod_{k=1}^{l_2}h_k
$$
is not identically zero.
\end{lemma}
\begin{proof}
Without loss of generality, assume $l_1 \le l_2$ and $q_1 < q_2$. Set $\zeta(B)=\sum_{E\in \calT_\calE}\chi(E)$, by collecting a common denominator, we then see that
  $$
  f(B)=\frac{a_1\zeta^{(l_2-l_1)}(B)\tilde{g}(B) + a_2\tilde{h}(B)}{\zeta^{l_2}(B)},
  $$
 where $\tilde{g}(B)$ and $\tilde{h}(B)$ are homogeneous polynomials in $B$ with order $l_1(n-1)$ and $l_2(n-1)$, respectively.
 
Let $\alpha(g):=(e_j: g_k=D_{e_i, e_j}, e_i\neq e_j, k =1,2,\cdots, l_1)$ be the vector collecting all edges $e_j$ corresponding to terms in $g_k$'s with $e_i\neq e_j$, and define $\alpha(h)$ similarly. Since $q_1 < q_2$, we can find an edge $\tilde{e}_j$ in $\alpha(h)$ that is not in $\alpha(g)$. Without loss of generality, say this specific $h$ is $h_{\tilde{k}}$.  By Lemma \ref{lemma:no_contain}, we know that the numerator of $h_{\tilde{k}}$ does not contain $B_{\tilde{e}_j}$. As a result, the order of $B_{\tilde{e}_j}$ is at most $l_2 - 1$ in all terms of $\tilde{h}(B)$.

Now, we claim that $\zeta^{(l_2-l_1)}(B)\tilde{g}(B)$ contains a term where $B_{\tilde{e}_j}$ is of order $l_2$, which is strictly larger than $l_2 - 1$. This term cannot be canceled by any term from $\tilde{h}(B)$, and thus we know $f(B)$ is not identically zero. To show this claim, note that by expanding $\zeta^{(l_2-l_1)}(B)\tilde{g}(B)$, we see that each term in $\zeta^{(l_2-l_1)}(B)\tilde{g}(B)$ is a product of terms from the factors involved. Thus it suffices to pick a term that contains $B_{\tilde{e}_j}$  from each of these factors.

First we consider the $\zeta$ factor. Since $\zeta$ sums over all spanning trees in $\calG$, and any edge in $\calG$ can be extended to a spanning tree of $\calG$ by iteratively adding edges, we know there exists at least one term in $\zeta$ that contains $B_{\tilde{e}_j}$. We pick this term out for every $\zeta$ in $\zeta^{(l_2-l_1)}(B)\tilde{g}(B)$, which multiplies to a term in which $B_{\tilde{e}_j}$ has order $l_2-l_1$.

Next, we consider $g_k$'s with $e_i=e_j$. For such $g_k$, since $e_i$ and $\tilde{e}_j$ are within the same cell, we can find a simple loop in this cell that contains both $e_i$ and $\tilde{e}_j$. Removing an edge different from $e_i$ and $\tilde{e}_j$ from this loop induces a path which, by iteratively adding edges, can be extended to a spanning tree that passes through $e_j$ and $\tilde{e}_j$. This tree is an element of $\calT_{e_i}$, and thus by Lemma \ref{lemma:contain} appears in the numerator of $g_k$. We pick this term for $g_k$, which contains $B_{\tilde{e}_j}$. Doing so for all $g_k$'s of this type contributes $l_1-q_1$ order of $B_{\tilde{e}_j}$.

Lastly, we consider $g_k$'s with $e_i\neq e_j$. Since $e_i$ and $\tilde{e}_j$ are within the same cell, we can find a simple loop in this cell that contains both $e_i$ and $\tilde{e}_j$. If $e_j$ is also in this loop, then we remove $e_j$. Otherwise, remove an edge different from $e_i$ and $\tilde{e}_i$. This induces a path that contains $e_i$ and $\tilde{e}_j$ but not $e_j$. By iteratively adding edges other than $e_j$, we can extend this path into a spanning tree of $\calG$ that contains $e_i$ and $\tilde{e}_j$ but not $e_j$, which in particular is an element of $\calT_{e_i, -e_j}$. By \eqref{eqn:local_exp_formula} we then know that this tree appears in the numerator of $g_k$. We pick this term for $g_k$, which contains $B_{\tilde{e}_j}$. Doing so for all $g_k$'s of this type contributes $q_1$ order of $B_{\tilde{e}_j}$.

In summary, we can find a term that contains $B_{\tilde{e}_j}$ in every factor of $\zeta^{(l_2-l_1)}(B)\tilde{g}(B)$. Multiplying all these terms together induces a term of $\zeta^{(l_2-l_1)}(B)\tilde{g}(B)$ where $B_{\tilde{e}_j}$ is of order $l_2$. Our claim then follows, and this completes the proof.
\end{proof}
Recall that
\begin{equation}\label{eqn:det_frobenious}
\det(J_1')=\sum_{\sigma\in \calS_{m_1-1}}\sgn(\sigma)\prod_{e}(J_1')_{e\sigma(e)},
\end{equation}
where $\calS_{m_1-1}$ is the symmetric group of order $m_1-1$ and $\sgn(\sigma)$ is the signature of $\sigma$.

Now, depending on whether $e_1=e_2$, the matrix $J'_1$ contains either $m_1-1$ or $m_1-2$ entries of the form $1-D_{\tilde{e}_i,\tilde{e}_j}$. When there are $m_1-1$ such entries, they must all appear on the diagonal of $J_1'$, and thus multiplying all these terms induces a term in \eqref{eqn:det_frobenious} that has the form
$$
\prod_{k=1}^{m_1-1}D_{e_{i_k},e_{i_k}}.
$$
All other terms in $\det(J_1')$ contain at least one factor of the form $D_{\tilde{e}_i, \tilde{e}_j}$ with $\tilde{e}_i\neq\tilde{e}_j$ (and hence at most $m_1-2$ factor of the form $D_{\tilde{e},\tilde{e}}$), and thus by Lemma \ref{lemma:non_vanishing}, cannot cancel the above term. As a result, we know that $\det(J_1')$ is not identically zero.

When there are $m_1-2$ entries of the form $1-D_{\tilde{e}_i,\tilde{e}_j}$ in $J_1'$, these entries must appear on the diagonal of $J_1'$. And thus multiplying them together with the remaining diagonal entry of $J_1'$ induces a term in \eqref{eqn:det_frobenious} that has exactly $m_1-2$ factors of the form $D_{\tilde{e},\tilde{e}}$. Meanwhile, all other terms in $\det(J_1')$ contain at least two factors of the form $D_{\tilde{e}_i, \tilde{e}_j}$ with $\tilde{e}_i\neq\tilde{e}_j$ (and hence at most $m_1-3$ factors of the form $D_{\tilde{e},\tilde{e}}$), and thus by Lemma \ref{lemma:non_vanishing}, cannot cancel the above term. As a result, $\det(J_1')$ is not identically zero.

In summary, we have shown that $\det(J_1')$ is a rational function that is not identically zero. Therefore,
$$
\mu(\det(J_1')=0)=\calL_m(\det(J_1')=0) = 0,
$$
or, equivalently, $(H_1)_{e_1e_2}\neq 0$ almost surely in $\mu$. \qed

==> multi_line_no_cut.tex <==


Without loss of generality, assume $e\in E_1$. Proposition \ref{prop:multi_line_label} implies that the $e$-th column of $B_{-E}C_{-E}^TAC_E(I-B_EC_E^TAC_E)^{-1}$ is given by
$$
B_{-E}C_{-E}^TAC_{E_1}(H_1)_e,
$$
where $(H_1)_e$ is the column of $H_1$ corresponding to the edge $e$. It then follows that
$$
K_{\hat{e}e}^{E}=\sum_{e'\in E_1}D_{\hat{e}, e'}(H_1)_{e' e}.
$$

From the proof of Proposition \ref{prop:multi_line_label}, we can rewrite the above formula to
\begin{equation}\label{eqn:trying_to_find_a_name}
K_{\hat e e}^{E}=\frac{\sum_{e'\in E_1}D_{\hat{e}, e'}\det(J_1^{e',e})}{\det(J_1)},
\end{equation}
where $J_1^{e',e}$ is the matrix obtained from $J_1$ by replacing the $e'$-th column with a vector with value $1$ at $e$-th component and $0$ elsewhere. 

If $\hat{e}\notin \calC_1$, then $D_{\hat{e}, e'}=0$ for all $e'\in E_1$ by Theorem \ref{thm:summary}. Thus we know $K_{\hat{e}e}^E=0$.

If $\hat{e}\in \calC_1$, then we claim that the numerator of \eqref{eqn:trying_to_find_a_name} is not identically zero. If the claim is true, then
$$\mu(K^E_{\hat{e}e}\neq0)=\calL_m(K^E_{\hat{e}e}\neq0)=1$$ and this completes the proof. 

We now show the claim indeed holds. First we consider the case $\hat{e}\notin E_1$. In this case, note that the term in \eqref{eqn:trying_to_find_a_name} corresponding to $e'=e$ contains one term that has exactly $m_1-1$ factors of the form $D_{\tilde{e}, \tilde{e}}$ ($\hat{e} \neq e'$ for all $e'\in E_1$ in this case), while all other terms in the numerator of \eqref{eqn:trying_to_find_a_name} contains at most $m_1-2$ factors of the form $D_{\tilde{e}, \tilde{e}}$. From Lemma \ref{lemma:non_vanishing} we then see that the numerator of \eqref{eqn:trying_to_find_a_name} is not identically zero.

Next we consider the case $\hat{e}\in E_1$ but $\hat{e}\neq e$. In this case, among all terms of \eqref{eqn:trying_to_find_a_name}, only the terms corresponding to $e'=\hat{e}$ and $e'=e$ contain one term that has exactly $m_1-1$ factors of the form $D_{\tilde{e}, \tilde{e}}$, and these two terms are
$$
D_{\hat{e},e}D_{\hat{e},\hat{e}}\prod_{e''\neq e,\hat{e}}D_{e'',e''}
$$
and
$$
D_{e,\hat{e}}D_{\hat{e},\hat{e}}\prod_{e''\neq e,\hat{e}}D_{e'',e''},
$$
respectively, which do not cancel each other since $\hat{e}\neq e$. All other terms in the numerator of \eqref{eqn:trying_to_find_a_name} contain at most $m_1-2$ factors of the form $D_{\tilde{e}, \tilde{e}}$. From Lemma \ref{lemma:non_vanishing} we then see that the numerator of \eqref{eqn:trying_to_find_a_name} is not identically zero.

Finally we consider the case $\hat{e}=e$. In this case, among all terms of \eqref{eqn:trying_to_find_a_name}, only the term corresponding to $e'=e$ contains one term that has exactly $m_1$ factors of the form $D_{\tilde{e}, \tilde{e}}$,  while all other terms in the numerator of \eqref{eqn:trying_to_find_a_name} contain at most $m_1-2$ factors of the form $D_{\tilde{e}, \tilde{e}}$. Lemma \ref{lemma:non_vanishing} then implies that the numerator of \eqref{eqn:trying_to_find_a_name} is not identically zero, which concludes the proof of the claim. \qed

==> non_bridge.tex <==
In this section, we % characterize power flow redistribution under the DC model when a single non-bridge line is tripped and
 show that the impacts of a single non-bridge line failure are localized within a tree-partition region. % More specifically, we study how the tripping of a line $e\in\calE$ impacts the branch flow on a different line $\hat{e}\in\calE$.
 Recall from Proposition 10 in Part I that $K_{\hat{e}e}$ is a precise indicator on whether the failure $e$ can potentially lead to the successive failure of line $\hat{e}$.

\subsection{Impact across Regions}
We consider first the case where $\hat{e}$ does not belong to the same region as $e$, that is, $\hat{e}$ either belongs to a different region or $\hat{e}$ is a bridge. 
\begin{prop}\label{prop:disjoint_island}
Consider a power network $\calG$ with a tree partition $\calP=\set{\calN_1,\calN_2,\cdots, \calN_k}$. Let $e, \hat{e}\in\calE$ be two different edges such that $e$ is not a bridge. Then $K_{\hat{e}e} = 0$ for any $\hat{e}$ that is not in the same region containing $e$.
\end{prop}
See \iftoggle{isreport}{Appendix \ref{proof:across_bridge}}{our online report \cite{part2}} for a proof. This result implies that, when a non-bridge line $e$ fails, any line $\hat{e}$ not in the same tree-partition region as $e$ will not be affected, regardless of whether $\hat{e}$ is a bridge. In other words, non-bridge failures cannot propagate through the boundaries formed by the tree-partition regions of $\calG$.

\subsection{Impact within Regions}
It is reasonable to expect that the converse to the above result is also true. That is, if $e, \hat{e}$ belong to the same region (and thus $e$ is not a bridge), we would expect $K_{\hat{e}e}\neq 0$. This, however, might not always be the case for two reasons: 1) some nodes within a tree-partition region may ``block'' simple loops containing both $e$ and $\hat{e}$; 2) the graph $\calG$ may be too symmetric. We elaborate on these two scenarios separately in the following two subsections.

\subsubsection{Block Decomposition}
The following example illustrates the situation in which nodes inside a tree-partition region may ``block'' simple loops containing both $e$ and $\hat{e}$.

\begin{figure}
\centering
\iftoggle{isarxiv}{
\subfloat[]{\includegraphics[height=2cm]{arxiv_figs/butterfly.eps}
}
\hfill
\subfloat[]{\includegraphics[height=2cm]{arxiv_figs/butterfly_decomp.eps}
}
}{
\subfloat[]{\includegraphics[height=1.6cm]{figs/butterfly.png}
}
\hfill
\subfloat[]{\includegraphics[height=1.6cm]{figs/butterfly_decomp.png}
}
}
\caption{(a) A butterfly network. (b) The block decomposition of the butterfly network into cells $\calC_1$ and $\calC_2$.}\label{fig:butterfly}
\end{figure}

\begin{eg}\label{eg:butterfly}
Consider the butterfly network shown in Fig.~\ref{fig:butterfly}(a) and pick $e=(i,j)$ and $\hat{e}=(w,z)$. It is not hard to see that any loop containing $e$ and $\hat{e}$ must pass through the central node $c$ at least twice and hence is never simple. The Simple Loop Criterion (Theorem 11 in \emph{\cite{part1}}) immediately yields that $K_{\hat{e}e}=0$. %\qedd
\end{eg}
The underlying issue in this example is that the butterfly network is not 2-connected, which means that the removal of a single node (in this case the central node $c$) can disconnect the original graph. Network nodes with such a property are referred to as \emph{cut vertices} in graph theory. As in Example \ref{eg:butterfly}, cut vertices prevent the existence of global simple loops.

Fortunately, we can precisely capture such an effect by decomposing each tree-partition region further through the classical \emph{block decomposition}~\cite{harary1969graph}. Recall that the block decomposition of a graph is a partition of its edge set $\calE$ such that each partitioned component is 2-connected, see Fig.~\ref{fig:butterfly}(b) for an illustration. The block decomposition of a graph always exists and can be found in linear time~\cite{tarjan1985efficient}. We refer to the components of this decomposition as \emph{cells} to reflect the fact that they are smaller parts within a tree-partition region. Note that two different cells within the same tree-partition region may share a common vertex, since the block decomposition induces a partition only of the network edges.

\begin{lemma}
\label{lemma:differentcells}
If $e,\hat{e}$ are two distinct edges within the same tree-partition region that belong to different cells, then $K_{\hat{e}e}=0$.
\end{lemma}
\begin{proof}
Let $\calC_e$ and $\calC_{\hat{e}}$ be the two cells to which $e$ and $\hat{e}$ respectively belong. It is a well-known result that any path from a node in $\calC_e$ to a node in $\calC_{\hat{e}}$ must pass through a common cut vertex in $\calC_e$ or $\calC_{\hat{e}}$ \cite{harary1969graph}. It is then impossible to find a simple loop containing both $e$ and $\hat{e}$ and, thus, the Simple Loop Criterion implies that $K_{\hat{e}e}=0$.
\end{proof}

\subsubsection{Symmetry}
Next, we show how graph symmetries (more specifically, graph automorphisms) may also block the propagation of failures. We first illustrate the issue by means of an example. 

\begin{eg}\label{eg:symmetry}
Consider the power network $\calG$ consisting of the complete graph on $n$ vertices ($n\ge 4$) and line susceptances all equal to $1$. Pick two edges $e=(i,j)$ and $\hat{e}=(w,z)$ that do not share any common endpoints. By symmetry, it is easy to see that there is a bijective correspondence between $\calT\paren{\set{i,w},\set{j,z}}$ and $\calT\paren{\set{i,z},\set{j,w}}$, and thus
$$
\sum_{E\in \calT(\set{i,w},\set{j,z})}\chi(E)-\sum_{E\in \calT(\set{i,z},\set{j,w})}\chi(E) = 0.
$$
By Theorem \ref{thm:redist_factor}, we then have $K_{\hat{e}e}=0$.
\end{eg}

A complete graph is 2-connected and thus consists of a single cell. Example \ref{eg:symmetry} shows that even if two edges $e,\hat{e}$ are within the same cell, when the graph $\calG$ is rich in symmetry, it is still possible that a failure of line $e$ does not impact another line $\hat{e}$. Nevertheless, this issue is not critical as such a symmetry almost never happens in practical systems, because of heterogeneity in line susceptances. In fact, even if the power network topology is highly symmetric, an infinitesimal change on the line susceptances is enough to break the symmetry, as we now show.

More specifically, we take the line susceptances to be average values $B_e$ plus
random perturbations $\omega=(\omega_e: e\in\calE)$ drawn from a probability measure $\mu$. Such perturbations can come from manufacturing error or measurement noise. The perturbed system\footnote{We assume the perturbation ensures $B_e+\omega_e > 0$ for any $e\in\calE$ so that the new susceptance is physically meaningful.} shares the same topology (and thus tree partition) as the original system, yet admits perturbed susceptances $B+\omega$. The randomness of $\omega$ implies the factors $K_{\hat{e}e}$ are now random variables. Recall that we assume $\mu$ to be \emph{absolutely continuous} with respect to Lebesgue measure $\calL_m$ on $\R^m$, which means that for any measurable set $S$ such that $\calL_m(S)=0$, we have $\mu(S)=0$.

\begin{prop}\label{prop:same_region}
Consider a power network $\calG$ with susceptance perturbation $\mu$ and let $e,\hat{e}$ be two distinct edges within the same cell. If $\mu$ is absolutely continuous with respect to $\calL_m$, then $K_{\hat{e}e}\neq 0$ $\mu$-\textit{almost surely}, i.e., $\mu\paren{K_{\hat{e}e}\neq 0} = 1$.
\end{prop}
\iftoggle{isreport}{See Appendix \ref{proof:same_region} for a proof.}{See our online report for a proof \cite{part2}.}
Note that, by the Radon-Nikodym Theorem~\cite{royden2010real}, the probability measure $\mu$ is absolutely continuous with respect to $\calL_m$ if and only if it affords a probability density function. This essentially amounts to requiring the measure $\mu$ to not contain Dirac masses. As a result, we see that for almost all relevant stochastic models on such perturbations (e.g.,~truncated Gaussian noise with arbitrary covariance, bounded uniform distribution, truncated Laplace distribution), the assumption applies and, thus, $K_{\hat{e}e}\neq 0$ for $e,\hat{e}$ within the same cell almost surely, no matter how small the perturbation is.\iftoggle{isreport}{\footnote{Our
results can be readily extended to the case when $\mu$ contains Dirac masses. See Appendix \ref{appendix:dirac} for more discussion.}}{}
%\lguo{Is this worth mentioning?}\slow{It's worthwhile to include at least for the arXiv version.}}. 

This perturbation approach is also useful for our results in the following sections. When we take this approach, our result often constitutes two directions: (a) an ``only if'' direction that should be interpreted as normal; and (b) an ``if'' direction that holds almost surely in $\mu$. To simplify the presentation, we henceforth fix an absolutely continuous perturbation $\mu$ with respect to  $\calL_m$, and define the following:
\begin{defn}\label{defn:mu_iff}
 For two predicates $p$ and $q$, we say that $p$ \textbf{\emph{``if'' and only if}} $q$ when both of the following hold:
$$
p\Ra q, \qquad q\Ra \mu(p)=1.
$$
\end{defn}
We say the ``if'' is in $\mu$-sense when we need to emphasize that the ``if'' direction only holds almost surely in $\mu$.

Proposition \ref{prop:disjoint_island}, Lemma \ref{lemma:differentcells}, 
and Proposition \ref{prop:same_region} prove the first half of Theorem \ref{thm:summary}.

==> preliminaries.tex <==
In this section, we present the cascading failure model that our main technical results build upon. This model extends the DC power flow model presented in Part I to multiple stages, and is a special case of the integrated failure propagation model that we introduce in Part III.

Given a power network, we describe the cascading failure process by keeping track of the set of failed lines at different stages indexed by $\mathfrak{N}:=\set{1,2,\cdots, N}$. Each stage $\mathfrak{n}\in\mathfrak{N}$ corresponds to a graph $\calG(\mathfrak{n}):=(\calN,\calE\bs\calB(\mathfrak{n}))$, where $\calB(\mathfrak{n})$ is the set of all tripped lines at stage $\n$ and is naturally nested:
$$
\calB(\mathfrak{n}) \subset \calB(\mathfrak{n}+1), \quad \forall \mathfrak{n} \in \mathfrak{N}.
$$
Within each stage $\n$, the power flow redistributes over the network described by $\calG(\n)$ according to the DC power flow model (see Part I for more details).   %After the system stabilizes, if
If all the branch flows are below the corresponding line ratings, then the new operating point is secure and the cascade stops. Otherwise, let $\calF(\n)$ be the subset of lines whose branch flows exceed the corresponding line ratings. The lines in $\calF(\n)$ are tripped in stage $\n$, i.e., $\calB(\n +1)=\calB(\n)\cup\calF(\n)$. This process repeats for stage $\n + 1$ and so on.

Next, we focus on a fixed stage $\n\in\mathfrak{N}$, and describe how a single line failure impacts the branch flows on remaining lines. To simplify the notation, we drop the stage index from symbols such as $\calG(\n)$ and simply write them as $\calG$. Recall that when a line $e$ is tripped from $\calG$, if the newly formed graph $\calG':=(\calN,\calE\bs\set{e})$ is still connected, then the branch flow change on a line $\hat{e}$ with the same power injections $p$ is given by
$
	\Delta f_{\hat{e}} = K_{\hat{e}e} f_e,
$
where $K_{\hat{e}e}$ is the line outage distribution factor (LODF) \cite{wood1996generation} from $e$ to $\hat{e}$. In Part I of this paper, by studying the transmission network Laplacian matrix, we derive a new formula for $K_{\hat{e}e}$ that precisely captures the Kirchhoff's Laws in terms of graphical structures. The new formula is replicated here for reference:
\begin{thm}\label{thm:redist_factor}
Let $e=(i,j), \hat{e}=(w,z) \in \calE$ be edges such that $\calG'=(\calN, \calE\bs\set{e})$ is connected. Then, $K_{\hat{e}e}$ is given by
\begin{equation*}
B_{\hat{e}}\times\frac{\sum_{E\in \calT(\set{i,w},\set{j,z})}\chi(E)-\sum_{E\in \calT(\set{i,z},\set{j,w})}\chi(E)}{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\chi(E)}.
\end{equation*}
\end{thm}
Theorem \ref{thm:redist_factor} allows us to check algebraic properties of $K_{\hat{e}e}$ by examining the network topology $\calG$. 
% In Part I, we showed 
Recall $K_{\hat{e}e} \neq 0$ means that the failure of $e$ can potentially lead to  
the failure of $\hat{e}$.
In Part I, we proved a \emph{Simple Loop Criterion}: $K_{\hat{e}e}\neq 0$ ``if'' and only if there exists a simple loop containing both $e$ and $\hat{e}$ in $\calG$. In particular, for two edges $e$ and $\hat{e}$ such that $e$ is not a bridge, if there is no simple loop containing both $e$ and $\hat{e}$, then $K_{\hat{e}e}=0$.

If the post-contingency graph $\calG'$ is disconnected, then it is possible that the original injections $p$ are no longer balanced in some connected components of $\calG'$. Thus, to compute the new power flows, a power balancing rule $\calR$ needs to be applied. Several such rules have been proposed and evaluated in the literature based on load shedding or generator response \cite{soltan2015analysis,bernstein2014power,bienstock2010n-k,bienstock2011control,bernstein2014vulnerability}. In this work, we do not specialize to any such rule but, instead, we identify key properties of these rules that guarantee our results to hold. For this reason, our more abstract approach allows us to characterize the power flow redistribution under a broad class of power balancing rules.

==> proofs_new.tex <==
\section{Proofs}\label{section:prem_proofs}
\subsection{Proof of Corollary \ref{cor:prem_cross_product}}\label{section:prem_proof_of_cross}
By Proposition \ref{prop:prem_basis}, we see that
\begin{IEEEeqnarray}{rCl}
&&\paren{\sum_{E\in \calT_\calE}\chi(E)}\paren{A_{iw} + A_{jz} - A_{iz} - A_{jw}} \nonumber\\
 &=&\sum_{E\in \calT(\set{i,w},\set{n})}\chi(E) + \sum_{E\in \calT(\set{j,z},\set{n})}\chi(E)\nonumber \\
 &&-\sum_{E\in \calT(\set{j,w},\set{n})}\chi(E) - \sum_{E\in \calT(\set{i,z},\set{n})}\chi(E)\label{eqn:prem_decomposed1}
\end{IEEEeqnarray}
We can decompose the set $\calT(\set{i,w},\set{n})$ based on the tree that the bus $j$ belongs to. This leads to the identity
$$
\calT(\set{i,w},\set{n})=\calT(\set{i,j,w},\set{n})\sqcup \calT(\set{i,w},\set{j,n}),
$$
where $\sqcup$ means disjoint union. Similarly we also have
$$
\calT(\set{j,z},\set{n})=\calT(\set{i,j,z},\set{n})\sqcup \calT(\set{j,z},\set{i,n})
$$
$$
\calT(\set{i,z},\set{n})=\calT(\set{i,j,z},\set{n})\sqcup \calT(\set{i,z},\set{j,n})
$$
$$
\calT(\set{j,w},\set{n})=\calT(\set{i,j,w},\set{n})\sqcup \calT(\set{j,w},\set{i,n})
$$
Plugging the above decompositions to \eqref{eqn:prem_decomposed1} and cancelling the common terms, we see
\begin{IEEEeqnarray}{rCl}
&&\paren{\sum_{E\in \calT_\calE}\chi(E)}\paren{A_{iw} + A_{jz} - A_{iz} - A_{jw}} \nonumber\\
 &=&\sum_{E\in \calT(\set{i,w},\set{j,n})}\chi(E) + \sum_{E\in \calT(\set{j,z},\set{i,n})}\chi(E)\nonumber\\
 &&-\sum_{E\in \calT(\set{j,w},\set{i,n})}\chi(E) - \sum_{E\in \calT(\set{i,z},\set{j,n})}\chi(E)\label{eqn:prem_decomposed2}
\end{IEEEeqnarray}
Again we have the following set identities
$$
\calT(\set{i,w},\set{j,n})=\calT(\set{i,w},\set{j,z,n})\sqcup\calT(\set{i,w,z},\set{j,n})
$$
$$
\calT(\set{j,z},\set{i,n})=\calT(\set{j,z},\set{i,w,n})\sqcup\calT(\set{j,w,z},\set{i,n})
$$
$$
\calT(\set{j,w},\set{i,n})=\calT(\set{j,w},\set{i,z,n})\sqcup\calT(\set{j,w,z},\set{i,n})
$$
$$
\calT(\set{i,z},\set{j,n})=\calT(\set{i,z},\set{j,w,n})\sqcup\calT(\set{i,w,z},\set{j,n})
$$
Plugging to \eqref{eqn:prem_decomposed2} and cancelling common terms, we see
\begin{IEEEeqnarray*}{rCl}
&&\paren{\sum_{E\in \calT_\calE}\chi(E)}\paren{A_{iw} + A_{jz} - A_{iz} - A_{jw}} \\
 &=&\sum_{E\in \calT(\set{i,w},\set{j,z,n})}\chi(E) + \sum_{E\in \calT(\set{j,z},\set{i,w,n})}\chi(E)\\
 &&-\sum_{E\in \calT(\set{j,w},\set{i,z,n})}\chi(E) - \sum_{E\in \calT(\set{i,z},\set{j,w,n})}\chi(E)\\
 &=&\sum_{E\in \calT(\set{i,w},\set{j,z})}\chi(E) - \sum_{E\in \calT(\set{j,w},\set{i,z})}\chi(E)
\end{IEEEeqnarray*}
where the last equality follows from
$$
\calT(\set{i,w},\set{j,z})=\calT(\set{i,w},\set{j,z,n})\sqcup \calT(\set{j,z},\set{i,w,n})
$$
and
$$
\calT(\set{j,w},\set{i,z})=\calT(\set{j,w},\set{i,z,n})\sqcup \calT(\set{i,z},\set{j,w,n}.
$$
\qed

\subsection{Proof of Lemma \ref{lemma:prem_l_a_equiv}}
To prove this result, we derive explicit formulae for the branch flow vector $f$ in terms of the power injection $p$. From $p=L\theta$ we know that whenever this equation is solvable, the solution $\theta$ is unique after quotienting away the kernel of $L$ given as $\spann\paren{\bff{1}}$. Noting this is also the kernel of $C^T$, we see that $f=BC^T\theta$ is uniquely determined. Towards the goal of an explicit formula, we can proceed in two ways. The first way relies on the fact that $L^\dagger p$ always gives a feasible $\theta$ and therefore
\begin{equation}\label{eqn:prem_pseudoinverse}
f=BC^TL^\dagger p
\end{equation}
The second way is to set the phase angle at the slack bus to zero, which implies that
$$
\ol{\theta}=\ol{L}^{-1}\ol{p} = A\ol{p}
$$
where $\ol{\theta}$ and $\ol{p}$ are the vector of non-slack bus phase angles and injections. Denote by $\ol{C}$ the matrix obtained from $C$ by removing the row corresponding to the slack bus. We then have
\begin{equation}\label{eqn:prem_submatrix}
f=B\ol{C}^T\ol{\theta}= B\ol{C}^TA \ol{p}.
\end{equation}
Now let $i, j \in\calN$ with neither $i$ nor $j$ being the slack bus. Under the injection $p_i=-p_j=1$, by equating the branch flow $f_{ij}$ computed from \eqref{eqn:prem_pseudoinverse} and \eqref{eqn:prem_submatrix}, we obtain that
$$
L^\dagger_{ii}+L^\dagger_{jj}-L^\dagger_{ij}-L^\dagger_{ji}=A_{ii}+A_{jj}-A_{ij}-A_{ji}.
$$
\qed

==> representation.tex <==
In this chapter, we present the main power grid model considered throughout the thesis and establish its basic properties that will be used in later chapters. In different applications, this model often needs to be augmented properly by adding more elements specific to the problem under study, and such augmentation will be presented in the relevant chapters.

\section{Laplacian Matrix}\label{section:prem_laplace}
The DC power flow equations \eqref{eqn:prem_dc} imply that
$$
p=CBC^T\theta.
$$
That is, the steady state phase angle $\theta$ is related to the steady state injection $p$ via the matrix $CBC^T$. This matrix is known as the Laplacian matrix of $\calG$ and plays a central role in all of our analysis in later chapters. We denote $L=CBC^T$ and present below some of its basic properties.

For any $v\in\R^n$, we can compute
\begin{equation}\label{eqn:prem_quadratic_form}
v^T Lv=\sum_{(i,j)\in\calE}B_{ij}(v_i-v_j)^2 \ge 0
\end{equation}
This immediately implies that
\begin{lemma}\label{lemma:prem_laplace_psd}
$L$ is positive semidefinite and hence diagonalizable.
\end{lemma}
Moreover, equation \eqref{eqn:prem_quadratic_form} attains equality if and only if $v_i=v_j$ for any $(i,j)\in\calE$. Since $L$ is symmetric, we then know\begin{lemma}\label{lemma:prem_laplace_kernel}
If $\calG$ is connected, then the kernel of $L$ is $\spann\paren{\bff{1}}$, the set of vectors with uniform entries.
\end{lemma}
This result tells us that the Laplacian matrix $L$ for a connected graph has rank $n-1$, where $n$ is the number of nodes, and hence $\det(L)=0$. A less obvious result, known as the Kirchhoff's Matrix Tree Theorem, states that (see \cite{chaiken1982allminor} for more details)
\begin{prop}\label{prop:prem_laplace_tree}
For any $i\in\calN$, let $L^{ii}$ be the matrix obtained from from $L$ by removing the $i$-th row and $i$-th column, then
$$
\det(L^{ii})=\sum_{E\in\calT}\prod_{e\in E}B_e
$$
where $\calT$ is the set of spanning trees on $\calG$.
\end{prop}
This result tells us that the matrix $L^{ii}$ is invertible. As we show in Section \ref{section:prem_inversion}, all elements of such matrices can be fully determined using proper ``tree distributions'' of $\calG$, and thus can be interpreted graphically.



\section{Graphical Interpretation of the Laplacian Inverse}\label{section:prem_inversion}
\begin{figure}
\centering
\includegraphics[scale=.5]{figs/spanning_forest}
\caption{An example element in $\calT(\calN_1,\calN_2)$, where circles correspond to elements in $\calN_1$ and squares correspond to elements in $\calN_2$. The two spanning trees containing $\calN_1$ and $\calN_2$ are highlighted as solid lines.}\label{fig:prem_spanning_forest}
\end{figure}

In this section, we explain how the inverse of $L^{ii}$ as defined in Proposition \ref{prop:prem_laplace_tree} is related to the ``tree distributions'' of the power network $\calG$. To simplify the notation, we fix the choice of $L^{ii}$ by picking $i$ to be the slack bus of $\calG$ (which without loss of generality is assumed to be the bus $n$), and denote the resulting matrix as $\ol{L}$. Put $A:=\ol{L}^{-1}$.

Given a subset $E$ of $\calE$, we use $\calT_E$ to denote the set of spanning trees of $\calG$ with edges from $E$. For two subsets $\calN_1, \calN_2$ of $\calN$, we define $\calT(\calN_1, \calN_2)$ to be the set of spanning forests of $\calG$ consisting of exactly two trees that contain $\calN_1$ and $\calN_2$ respectively. See Fig.~\ref{fig:prem_spanning_forest} for an illustration of $\calT(\calN_1, \calN_2)$. Given a set $E$ of edges, we write
$$
\chi(E):=\prod_{e\in E}B_e
$$
Then the celebrated All Minors Matrix Tree Theorem \cite{chaiken1982allminor} applied to the matrix $\ol{L}$ implies:
\begin{prop}\label{prop:prem_all_minor}
  The determinant of the matrix obtained by deleting the $i$-th row and $j$-th column of $\ol{L}$, denoted as $\ol{L}^{ij}$, is given by
  $$
  \det\paren{\ol{L}^{ij}}=(-1)^{i+j}\sum_{E\in \calT(\set{i,j},\set{n})}\chi(E)
  $$
\end{prop}
This result leads to the following graphical interpretation of the matrix $A$:
\begin{prop}\label{prop:prem_basis}
  For any $i,j\in\calN$ that are not slack buses, we have
  $$
  A_{ij}=\frac{\sum_{E\in \calT(\set{i,j},\set{n})}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)}
  $$
\end{prop}
\begin{proof}
Put $A_j$ to be the $j$-th column of $A$. Note that $\ol{L}A_{j}=e_j$. Therefore by Cramer's rule, we have
$$
A_{ij}=\frac{\det\paren{\ol{L}^i_j}}{\det\paren{\ol{L}}}
$$
where $\ol{L}^i_j$ is the matrix obtained by replacing the $i$-th column of $\ol{L}$ by $e_j$. Now by Proposition \ref{prop:prem_all_minor}, we have
$$
\det\paren{\ol{L}^i_j}=(-1)^{i+j}\det{\ol{L}^{ij}}=\sum_{E\in \calT(\set{i,j},\set{n})}\chi(E)
$$
and by Kirchhoff's Matrix Tree Theorem \cite{chaiken1982allminor}
$$
\det\paren{\ol{L}}=\sum_{E\in \calT_\calE}\chi(E).
$$
The desired result then follows.
\end{proof}
The following corollary is an interesting implication of Proposition \ref{prop:prem_basis}:
\begin{cor}
For all $i,j\in\calN$ that are different from the slack bus, we have
$$
A_{ij} \ge 0,
$$
where the equality holds if and only if every path from $i$ to $j$ contains $n$.
\end{cor}
\begin{proof}
Since $\chi(E) \ge 0$ for all $E$, we clearly have $A_{ij} \ge 0$ and equality holds if and only if the set $\calT(\set{i,j},\set{n})$ is empty.

If every path from $i$ to $j$ contains $n$, then since any tree containing $\set{i,j}$ induces a path from $i$ to $j$, we know that this tree also contains $n$. As a result, $\calT(\set{i,j}, \set{n}) = \emptyset$. Conversely, if $\calT(\set{i,j}, \set{n}) = \emptyset$, then any path from $i$ to $j$ must contain $n$, since for any path from $i$ to $j$ not passing $n$, we can iteratively add edges that do not have $n$ as an endpoint to obtain a spanning tree over the nodes set $\calN\bs \set{n}$. This tree together with the node $n$ itself is an element of $\calT(\set{i,j}, \set{n})$.

We thus have shown that $\calT(\set{i,j},\set{n})$ is empty if and only if every path from $i$ to $j$ contains $n$. This completes the proof.
\end{proof}
 
As another application of Proposition \ref{prop:prem_basis}, we now derive an alternative formula for the generation shift sensitivity factor \cite{wood1996generation}, that is widely studied in power system analysis literature and is defined as follows: For a pair of buses $i,j$ and an edge $e=(w,z)$, suppose we shift injection of amount $\delta p$ from $i$ to $j$, then the branch flow on $e$ changes accordingly by the DC power flow equations \eqref{eqn:prem_dc}. Denote such branch flow change by $\delta f_e$. The generation shift sensitivity factor between the pair of buses $i,j$ and the edge $e$ is defined to be the ratio between such changes:
$$
D_{ij,e}:=\frac{\delta f_e}{\delta p}
$$
Under DC power flow \eqref{eqn:prem_dc}, $D_{ij,e}$ is fully determined by the matrix $A$, and can be computed as (see \cite{wood1996generation}):
$$
D_{ij,e} = A_{iw} + A_{jz} - A_{iz}- A_{jw}
$$
\begin{cor}\label{cor:prem_cross_product}
  For $i,j,w,z\in\calN$ that are different from the slack bus, we have
  \begin{IEEEeqnarray*}{rCl}
  A_{iw} + A_{jz} - A_{iz}- A_{jw} &=&\frac{1}{\sum_{E\in \calT_\calE}\chi(E)}
  \paren{\sum_{E\in \calT(\set{i,w},\set{j,z})}\chi(E)-\sum_{E\in \calT(\set{i,z},\set{j,w})}\chi(E)}
  \end{IEEEeqnarray*}
\end{cor}
Note that this result holds regardless of whether $(w,z)$ is an edge in $\calE$ or not. Please refer to Section \ref{section:prem_proofs} for its proof.

Corollary \ref{cor:prem_cross_product} tells us that the impact of shifting generations from $i$ to $j$ propagates to the edge $e=(w,z)$ through trees that connect these endpoints. It suggests an interesting observation that, if such trees can be prevented from being formed, we can in fact ``eliminate'' the impact of the generation shift from $i$ to $j$ on the edge $e$. This observation, when interpreted in a different setting, motivates all of our results in disruption localization in Chapter \ref{chapter:localizability}.

As a concluding example, we derive a result using Corollary \ref{cor:prem_cross_product} that relates the effective reactance $R_{ij}$ introduced in Section \ref{section:prem_laplace} to the ``tree distributions'' of $\calG$. To do so, we need the following relation between $L^\dagger$ and $A$, which is also proved in Section \ref{section:prem_proofs}:
\begin{lemma}\label{lemma:prem_l_a_equiv}
For $(i,j)\in\calE$ such that $i\neq n$, $j\neq n$, we have
$$
L^\dagger_{ii}+L^\dagger_{jj}-L^\dagger_{ij}-L^\dagger_{ji}=A_{ii}+A_{jj}-A_{ij}-A_{ji}
$$
\end{lemma}
In other words, we can replace the $L^{\dagger}$'s in \eqref{eqn:prem_effective_reactance} by the matrix $A$. 
\begin{cor}\label{cor:prem_effective_reactance}
For $(i,j)\in\calE$ such that $i\neq n$, $j\neq n$, we have
  $$
 X_{ij}-R_{ij}=X_{ij}\cdot\frac{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)}
  $$
  In particular, we always have $X_{ij}\ge R_{ij}$ and the inequality is strict if the graph after removing $(i,j)$ is connected.
\end{cor}
\begin{proof}

By taking $w=i$, $z=j$ in Corollary \ref{cor:prem_cross_product} and applying Lemma \ref{lemma:prem_l_a_equiv}, we see that
$$
R_{ij}=A_{ii}+A_{jj}-2A_{ij}=\frac{\sum_{E\in\calT(\set{i},\set{j})}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)}
$$
For each forest in $\calT(\set{i},\set{j})$, we can add the edge $(i,j)$ to form a spanning tree passing through $(i,j)$. Conversely, each spanning tree passing through $(i,j)$ after removing the edge $(i,j)$ produces a forest in $\calT(\set{i},\set{j})$. This by the definition of $\chi(E)$ implies
$$
\sum_{E\in\calT(\set{i},\set{j})}\chi(E)=X_{ij}\sum_{E\in\calT'}\chi(E)
$$
where $\calT'$ denotes the set of all spanning trees passing through $(i,j)$. This implies
\begin{IEEEeqnarray*}{rCl}
X_{ij}-R_{ij}&=&X_{ij}\cdot\frac{\sum_{E\in \calT_\calE}\chi(E)-\sum_{E\in\calT'}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)}\\
&=&X_{ij}\cdot\frac{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)}
\end{IEEEeqnarray*}
\end{proof}

This result tells us that for an edge $(i,j)$, the reduction ratio of its reactance coming from the network is precisely the (weighted) portion of spanning trees not passing through $(i,j)$ among all spanning trees. Thus more connections from the network leads to more reduction in the effective reactance on $(i,j)$, which agrees with our physical intuition.

We remark that this reactance reduction ratio is closely related to the spanning tree centrality measure \cite{teixeira2013spanning}. Indeed, from the very definition of spanning tree centrality, we have
$$
\frac{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)} + c_{(i,j)} = 1
$$
where $c_{(i,j)}$ denotes the spanning tree centrality of $(i,j)$. As a result,
$$
R_{ij} = X_{ij}c_{(i,j)}
$$
or in other words, in a power redistribution setting, the spanning tree centrality of a line precisely captures the ratio between its effective reactance and its physical line reactance. 



==> same_region_proof.tex <==
Let $\calC$ be the cell that $e$ and $\hat{e}$ belong to and write $e=(i,j)$ and $\hat{e}=(w,z)$. Consider the polynomial $f(B)$ with line susceptances $B=(B_e:e\in\calE)$ as variables given by
$$
f(B):=\sum_{E\in\calT\paren{\set{i,w}, \set{j,z}}}\chi(E)-\sum_{E\in\calT\paren{\set{i,z}, \set{j,w}}}\chi(E).
$$
We claim that $f$ is not identically zero.

First, let $C$ be a simple cycle in $\calC$ that contains both $e$ and $\hat{e}$. Such a cycle always exists as $\calC$ is 2-connected by construction, and it is a classical result that any pair of edges are contained in a simple cycle for 2-connected graphs \cite{harary1969graph}. Therefore, we can find two disjoint paths $P_1$ and $P_2$ connecting the endpoints of $e$ and $\hat{e}$. Without loss of generality, assume $P_1$ connects $i$ to $w$ and $P_2$ connects $j$ to $z$. By iteratively adding edges from $\calG$ to $P_1$ and $P_2$, we can extend $P_1$ and $P_2$ to a spanning forest of $\calG$ consisting of exactly two trees. Moreover, the tree extended from $P_1$ contains $\set{i, w}$ and the tree extended from $P_2$ contains $\set{j,z}$. Thus we have constructed an element of $\calT\paren{\set{i,w}, \set{j,z}}$. Denote this element by $E_0$.

Second, we show that 
$$\calT\paren{\set{i,w}, \set{j,z}}\cap \calT\paren{\set{i,z}, \set{j,w}}=\emptyset.$$
Indeed, consider an element $E_1$ from $\calT\paren{\set{i,w}, \set{j,z}}$, which consists of two trees $\calT_1$ and $\calT_2$ with $\calT_1$ containing $\set{i,w}$ and $\calT_2$ containing $\set{j,z}$. If $E_1\in\calT\paren{\set{i,z}, \set{j,w}}$, then $\calT_1$ must also contain $z$. However, this implies $z\in \calT_1\cap \calT_2$, and thus $\calT_1$ and $\calT_2$ are not disjoint, contradicting the definition of $\calT\paren{\set{i,w}, \set{j,z}}$.

As a result, we see that the element $E_0$ constructed in our first step contributes a term to $\sum_{E\in\calT\paren{\set{i,w}, \set{j,z}}}\chi(E)$ but not to $\sum_{E\in\calT\paren{\set{i,z}, \set{j,w}}}\chi(E)$. Therefore $f(B)$ contains non-vanishing terms and is not identically zero.

It is well-known from algebraic geometry that the root set of a polynomial which is not identically zero has Lebesgue measure zero \cite{federer1969geometric}. That is, we have
$$
\mu\paren{f(B+\omega)=0} = \calL_m\paren{f(B+\omega)=0} = 0,
$$
where the first equality is because $\mu$ is absolutely continuous with respect to $\calL_m$ (it is clear that the root set of the polynomial $f$ is measurable since $f$ is continuous).

Finally, by Theorem \ref{thm:redist_factor}, $K_{\hat{e}e}= 0$ if and only if $f(B+\omega)=0$. This fact implies that
$$
\mu(K_{\hat{e}e}\neq 0) = 1 - \mu(K_{\hat{e}e}=0) = 1-\mu\paren{f(B+\omega)=0} = 1
$$
and completes our proof. \qed

==> summary.tex <==
%\slow{Edit later.  Summarize Part I for Part II.}
%\cliang{Skip for now.}

\begin{comment}
\begin{thm}\label{thm:redist_factor}
Let $\hat{l}=(\hat i,\hat j), \hat{e}=(\hat{i},\hat{j}) \in \calE$ be edges such that $\calG'=(\calN, \calE\bs\set{e})$ is connected. Then, $K_{\hat{e}e}$ is given by
\begin{equation*}
B_{\hat{e}}\times\frac{\sum_{E\in \calT(i\hat{i},j\hat{j})}\beta(E)-\sum_{E\in \calT(i\hat{j},j\hat{i})}\beta(E)}{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\beta(E)}.
\end{equation*}
\end{thm}
\end{comment}
%\ale{Unresolved notation consistency check between Part I and II: we used the $\hat l, l$ notation in place of $\hat e, e$ in Part I.}


%Therefore, this result implies that, for essentially all networks of interest, the tree partition encodes rich information on how the failure of a line propagates through the network. 
%Therefore the conditions posed in Theorem \ref{thm:summary} are mostly for analytical rigor and they can usually be ignored in practical applications of our results.

%From Fig.~\ref{fig:matrix_block}, we see that compared to a full mesh transmission network consisting of single cell, it can be beneficial to switch off certain lines so that more regions/cells are created and the impact of line failures are more localized. We elaborate on this observation and its implications on practical systems in Section \ref{section:case_study}.



%The next two sections are devoted to the proof of Theorem \ref{thm:summary}. We first characterize power redistribution after the tripping of a single non-bridge line in Section \ref{section:non-bridge}, and then consider in Section \ref{section:bridge} the failure of a single bridge. In Section \ref{section:multi_line}, we generalize our single-line failure characterization to the case of multi-line failures.

